Quantitative Diffractometric Biosensing

Diffractometric biosensing is a promising technology to overcome critical limitations of refractometric biosensors, the dominant class of label-free optical transducers. These limitations manifest themselves by higher noise and drifts due to insufficient rejection of refractive index fluctuations caused by variation in temperature, solvent concentration, and most prominently, non-specific binding. Diffractometric biosensors overcome these limitations with inherent self-referencing on the submicron scale with no compromise on resolution. Despite this highly promising attribute, the field of diffractometric biosensors has only received limited recognition. A major reason is the lack of a general quantitative analysis. This hinders comparison to other techniques and amongst different diffractometric biosensors. For refractometric biosensors, on the other hand, such a comparison is possible by means of the refractive index unit (RIU). In this publication, we suggest the coherent surface mass density, $\Gamma_{\rm{coh}}$, as a quantity for label-free diffractometric biosensors with the same purpose as RIU in refractometric sensors. It is easy to translate $\Gamma_{\rm{coh}}$ to the total surface mass density $\Gamma_{\rm{tot}}$, which is an important parameter for many assays. We provide a generalized framework to determine $\Gamma_{\rm{coh}}$ for various diffractometric biosensing arrangements which enables quantitative comparison. Additionally, the formalism can be used to estimate background scattering in order to further optimize sensor configurations. Finally, a practical guide with important experimental considerations is given to enable readers of any background to apply the theory. Therefore, this paper provides a powerful tool for the development of diffractometric biosensors and will help the field to mature and unveil its full potential.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
